Thermodynamics and efficiency of sequentially collisional Brownian particles: The role of drivings

Brownian particles placed sequentially in contact with distinct thermal reservoirs and subjected to external driving forces are promising candidates for the construction of reliable thermal engines. In this contribution, we address the role of driving forces for enhancing the machine performance. Analytical expressions for thermodynamic quantities such as power output and efficiency are obtained for general driving schemes. A proper choice of these driving schemes substantially increases both power output and efficiency and extends the working regime. Maximizations of power and efficiency, whether with respect to the strength of the force, driving scheme or both have been considered and exemplified for two kind of drivings: a generic power-law and a periodically drivings.

==> eqs.tex <==
\begin{equation}
  \int_{0}^{\tau /2} X_{1} e^{\gamma  x} \left(\frac{2 x}{\tau }\right)^{\alpha } dx = 2^{\alpha } X_{1} \tau  (-\gamma  \tau )^{-\alpha -1} (\Gamma (\alpha +1)-\Gamma (\alpha +1,-t \gamma ))
\end{equation}

\begin{equation}
 \int_{\tau /2}^{\tau} X_{2} \left(1-\frac{2 x}{\tau }\right)^{\beta } e^{\gamma  \left(x-\frac{\tau }{2}\right)} dx = -X_{2} \left(2-\frac{4 t}{\tau }\right)^{\beta } (\gamma  (\tau -2 t))^{-\beta } \left(\beta  \Gamma (\beta )-\Gamma \left(\beta +1,\frac{1}{2} \gamma  (\tau -2 t)\right)\right)\gamma 
\end{equation}

\begin{equation}
\begin{split}
  \expval{v_{0}} &= \frac{2^{\alpha } X_{1} e^{\tau } (-\tau )^{-\alpha } \Gamma (\alpha +1)}{e^{\tau }-1}-\frac{2^{\alpha } X_{1} (-\tau )^{-\alpha } \Gamma (\alpha +1)}{e^{\tau }-1}+\frac{2^{\alpha } X_{1} (-\tau )^{-\alpha } \Gamma \left(\alpha +1,-\frac{\tau }{2}\right)}{e^{\tau }-1}\\
  &  -\frac{2^{\alpha } X_{1} e^{\tau } (-\tau )^{-\alpha } \Gamma (\alpha +1,0)}{e^{\tau }-1}-\frac{(-2)^{\beta } \beta  X_{2} e^{\tau /2} (-\tau )^{-\beta } \Gamma (\beta )}{e^{\tau }-1}+\frac{(-2)^{\beta } X_{2} e^{\tau /2} (-\tau )^{-\beta } \Gamma \left(\beta +1,-\frac{\tau }{2}\right)}{e^{\tau }-1}
\end{split}
\end{equation}


\begin{equation}
  v_{1}(t) = a_{1} + a_{2} + a_{3} + a_{4} + a_{5} + a_{6}
\end{equation}

where
\begin{equation}
    a_{1} = -\frac{2^{\alpha } X_{1} (-\tau )^{-\alpha } \Gamma (\alpha +1) e^{\tau -t}}{e^{\tau }-1}
\end{equation}
\begin{equation}
    a_{2} = -\frac{(-2)^{\beta } X_{2} (-\tau )^{-\beta } \Gamma (\beta +1) e^{\frac{\tau }{2}-t}}{e^{\tau }-1}
\end{equation}
\begin{equation}
    a_{3} = -\frac{2^{\alpha } X_{1} e^{-t} (-\tau )^{-\alpha } \Gamma (\alpha +1,-t)}{e^{\tau }-1}
\end{equation}
\begin{equation}
    a_{4} = +\frac{2^{\alpha } X_{1} (-\tau )^{-\alpha } e^{\tau -t} \Gamma (\alpha +1,-t)}{e^{\tau }-1}
\end{equation}
\begin{equation}
    a_{5} = +\frac{2^{\alpha } X_{1} e^{-t} (-\tau )^{-\alpha } \Gamma \left(\alpha +1,-\frac{\tau }{2}\right)}{e^{\tau }-1}
\end{equation}
\begin{equation}
    a_{6} = +\frac{(-2)^{\beta } X_{2} (-\tau )^{-\beta } e^{\frac{\tau }{2}-t} \Gamma \left(\beta +1,-\frac{\tau }{2}\right)}{e^{\tau }-1}
\end{equation}

\begin{equation}
  v_{2}(t) = b_{1} + b_{2} + b_{3} + b_{4} + b_{5} + b_{6}
\end{equation}

where
\begin{equation}
    b_{1} = -\frac{2^{\alpha } X_{1} \tau ^{-\alpha } \Gamma (\alpha +1) e^{-i \pi  \alpha -t+\tau }}{e^{\tau }-1}
\end{equation}
\begin{equation}
    b_{2} = -\frac{2^{\beta } \beta  X_{2} \tau ^{-\beta } \Gamma (\beta ) e^{\frac{3 \tau }{2}-t}}{e^{\tau }-1}
\end{equation}
\begin{equation}
    b_{3} = +\frac{2^{\alpha } X_{1} \tau ^{-\alpha } \Gamma \left(\alpha +1,-\frac{\tau }{2}\right) e^{-i \pi  \alpha -t+\tau }}{e^{\tau }-1}
\end{equation}
\begin{equation}
    b_{4} = +\frac{2^{\beta } X_{2} \tau ^{-\beta } e^{\frac{\tau }{2}-t} \Gamma \left(\beta +1,-\frac{\tau }{2}\right)}{e^{\tau }-1}
\end{equation}
\begin{equation}
    b_{5} = -\frac{2^{\beta } X_{2} \tau ^{-\beta } e^{\frac{\tau }{2}-t} \Gamma \left(\beta +1,\frac{1}{2} (\tau -2 t)\right)}{e^{\tau }-1}
\end{equation}
\begin{equation}
    b_{6} = +\frac{2^{\beta } X_{2} \tau ^{-\beta } e^{\frac{3 \tau }{2}-t} \Gamma \left(\beta +1,\frac{1}{2} (\tau -2 t)\right)}{e^{\tau }-1}
\end{equation}


\begin{align}
  W_{1} &= - \frac{1}{\tau} \int_{0}^{\tau/2}    X_1 \left( \frac{2 t}{\tau} \right)^{\alpha} \left( v_{1}(t) \right) dt \\
  &= - \frac{1}{\tau} \int_{0}^{\tau/2}    X_1 \left( \frac{2 t}{\tau} \right)^{\alpha} \left( a_{1} + a_{2} + a_{3} + a_{4} + a_{5} + a_{6} \right) dt \\
  &= W_{1}^{(\text{term1})} + W_{1}^{(\text{term2})} + W_{1}^{(\text{term3})} + W_{1}^{(\text{term4})} + W_{1}^{(\text{term5})} + W_{1}^{(\text{term6})}
\end{align}

where 

\begin{equation}
    W_{1}^{(\text{term3})} = -\frac{4^{\alpha } X_{1}^2 (-\tau )^{-\alpha } \tilde{X} }{\left(1-e^{\tau }\right) \tau }
\end{equation}
%\left(\frac{2^{-2 \alpha -3} (-\tau )^{\alpha +2} \, _2F_2\left(1,2 \alpha +2;\alpha +2,2 \alpha +3;-\frac{\tau }{2}\right)}{(\alpha +1)^2}+\frac{\pi  \tau ^{-\alpha } \csc (\pi  \alpha ) \left(\Gamma \left(\alpha +1,\frac{\tau }{2}\right)-\Gamma (\alpha +1)\right)}{\Gamma (-\alpha )}\right)
\begin{equation}
    W_{1}^{(\text{term4})} = -\frac{4^{\alpha } X_{1}^2 e^{\tau } (-\tau )^{-\alpha } \tilde{X}}{\left(e^{\tau }-1\right) \tau }
\end{equation}
%\left(\frac{2^{-2 \alpha -3} (-\tau )^{\alpha +2} \, _2F_2\left(1,2 \alpha +2;\alpha +2,2 \alpha +3;-\frac{\tau }{2}\right)}{(\alpha +1)^2}+\frac{\pi  \tau ^{-\alpha } \csc (\pi  \alpha ) \left(\Gamma \left(\alpha +1,\frac{\tau }{2}\right)-\Gamma (\alpha +1)\right)}{\Gamma (-\alpha )}\right)
\begin{equation}
    W_{1}^{(\text{term1})} = \frac{4^{\alpha } X_{1}^2 e^{\tau } \left(-\tau ^2\right)^{-\alpha } \Gamma (\alpha +1) \left(\Gamma (\alpha +1)-\Gamma \left(\alpha +1,\frac{\tau }{2}\right)\right)}{\left(e^{\tau }-1\right) \tau }
\end{equation}

\begin{equation}
    W_{1}^{(\text{term5})} = -\frac{4^{\alpha } X_{1}^2 \left(-\tau ^2\right)^{-\alpha } \Gamma \left(\alpha +1,-\frac{\tau }{2}\right) \left(\Gamma (\alpha +1)-\Gamma \left(\alpha +1,\frac{\tau }{2}\right)\right)}{\left(e^{\tau }-1\right) \tau }
\end{equation}

\begin{equation}
    W_{1}^{(\text{term2})} = \frac{(-1)^{\beta +2} X_{1} X_{2} e^{\tau /2} 2^{\alpha +\beta } \tau ^{-\alpha -1} (-\tau )^{-\beta } \Gamma (\beta +1) \left(\Gamma (\alpha +1)-\Gamma \left(\alpha +1,\frac{\tau }{2}\right)\right)}{e^{\tau }-1}
\end{equation}

\begin{equation}
    W_{1}^{(\text{term6})} = \frac{(-1)^{\beta +1} X_{1} X_{2} e^{\tau /2} 2^{\alpha +\beta } \tau ^{-\alpha -1} (-\tau )^{-\beta } \Gamma \left(\beta +1,-\frac{\tau }{2}\right) \left(\Gamma (\alpha +1)-\Gamma \left(\alpha +1,\frac{\tau }{2}\right)\right)}{e^{\tau }-1}
\end{equation}
%

%
\begin{align}
  W_{2} &= - \frac{1}{\tau} \int_{\tau/2}^{\tau}  X_2 \left(1-\frac{2t}{\tau}\right)^{\beta}  \left( v_{2}(t) \right) dt\\
  &= - \frac{1}{\tau} \int_{\tau/2}^{\tau}  X_2 \left(1-\frac{2t}{\tau}\right)^{\beta}  \left( b_{1} + b_{2} + b_{3} + b_{4} + b_{5} + b_{6} \right) dt\\
  &= W_{2}^{(\text{term1})} + W_{2}^{(\text{term2})} + W_{2}^{(\text{term3})} + W_{2}^{(\text{term4})} + W_{2}^{(\text{term5})} + W_{2}^{(\text{term6})}
\end{align}

where
\begin{equation}
    W_{2}^{(\text{term1})} = e^{-i \pi  \alpha } (-1)^{\beta +2} X_{1} X_{2} 2^{\alpha +\beta -1} \Gamma (\alpha +1) \text{csch}\left(\frac{\tau }{2}\right) \tau ^{-\alpha -\beta -1} \left(\Gamma (\beta +1)-\Gamma \left(\beta +1,\frac{\tau }{2}\right)\right)
\end{equation}
\begin{equation}
    W_{2}^{(\text{term2})} = \frac{(-4)^{\beta } \beta  X_{2}^2 e^{\tau } \tau ^{-2 \beta -1} \Gamma (\beta ) \left(\Gamma (\beta +1)-\Gamma \left(\beta +1,\frac{\tau }{2}\right)\right)}{e^{\tau }-1}
\end{equation}
\begin{equation}
    W_{2}^{(\text{term3})} = e^{-i \pi  \alpha } (-1)^{\beta +1} X_{1} X_{2} 2^{\alpha +\beta -1} \text{csch}\left(\frac{\tau }{2}\right) \tau ^{-\alpha -\beta -1} \Gamma \left(\alpha +1,-\frac{\tau }{2}\right) \left(\Gamma (\beta +1)-\Gamma \left(\beta +1,\frac{\tau }{2}\right)\right)
\end{equation}
\begin{equation}
    W_{2}^{(\text{term4})} = -\frac{(-4)^{\beta } X_{2}^2 \tau ^{-2 \beta -1} \Gamma \left(\beta +1,-\frac{\tau }{2}\right) \left(\Gamma (\beta +1)-\Gamma \left(\beta +1,\frac{\tau }{2}\right)\right)}{e^{\tau }-1}
\end{equation}
\begin{equation}
    W_{2}^{(\text{term5})} = \int_{\tau/2}^{\tau} -\frac{2^{\beta } X_{2}^2 \tau ^{-\beta } e^{\frac{\tau }{2}-t} \left(1-\frac{2 t}{\tau }\right)^{\beta } \Gamma \left(\beta +1,\frac{1}{2} (\tau -2 t)\right)}{e^{\tau }-1} dt
\end{equation}
\begin{equation}
    W_{2}^{(\text{term6})} = \int_{\tau/2}^{\tau} \frac{2^{\beta } X_{2}^2 \tau ^{-\beta } e^{\frac{3 \tau }{2}-t} \left(1-\frac{2 t}{\tau }\right)^{\beta } \Gamma \left(\beta +1,\frac{1}{2} (\tau -2 t)\right)}{e^{\tau }-1} dt
\end{equation}
%

\begin{align}
    C_{n}^{(1)}(t) &= \int_{0}^{t}e^{\gamma t'} \cos(\frac{4\pi n}{\tau} t') dt' \\
    \overline{C}_{n}^{(1)}(t) &= \int_{0}^{t}e^{-\gamma t'} \cos(\frac{4\pi n}{\tau} t') dt' \\
    S_{n}^{(1)}(t) &= \int_{0}^{t}e^{\gamma t'} \sin(\frac{4\pi n}{\tau} t') dt' \\
    \overline{S}_{n}^{(1)}(t) &= \int_{0}^{t}e^{-\gamma t'} \sin(\frac{4\pi n}{\tau} t') dt' \\
     C_{n}^{(2)}(t) &= \int_{\tau/2}^{t}e^{\gamma (t'-\tau/2)} \cos(\frac{4\pi n}{\tau} t') dt' \\
     \overline{C}_{n}^{(2)}(t) &= \int_{\tau/2}^{t}e^{-\gamma (t'-\tau/2)} \cos(\frac{4\pi n}{\tau} t') dt' \\
     S_{n}^{(2)}(t) &= \int_{\tau/2}^{t}e^{\gamma (t'-\tau/2)} \sin(\frac{4\pi n}{\tau} t') dt' \\
     \overline{S}_n^{(2)}(t) &= \int_{\tau/2}^{t}e^{-\gamma (t'-\tau/2)} \sin(\frac{4\pi n}{\tau} t') dt' 
\end{align}


